QAware: A Cross-Layer Approach to MPTCP Scheduling

Multipath TCP (MPTCP) allows applications to transparently use all available network interfaces by creating a TCP subflow per interface. One critical component of MPTCP is the scheduler that decides which subflow to use for each packet. Existing schedulers typically use estimates of end-to-end path properties, such as delay and bandwidth, for making the scheduling decisions. In this paper, we show that these scheduling decisions can be significantly improved by incorporating readily available local information from the device driver queues in the decision-making process. We propose QAware, a novel cross-layer approach for MPTCP scheduling. QAware combines end-to-end delay estimates with local queue buffer occupancy information and allows for a better and faster adaptation to the network conditions. This results in more efficient use of the available resources and considerable gains in aggregate throughput. We present the design of QAware and evaluate its performance through simulations, and also through real experiments, comparing it to existing schedulers. Our results show that QAware performs significantly better than other available approaches for various use-cases and applications.

==> discussion.tex <==
\section{Discussion and Future Work}\label{sec:discussion}

%\begin{table}[!tb]
%\centering
%\scalebox{0.75}{
%\begin{tabular}{@{}ccc@{}}
%\toprule
%\textbf{Host Machine}  & \textbf{Network}        & \textbf{Receiver}      \\ \midrule
%Data rate  & Channel utilization     & Bandwidth utilization  \\
%Retry percentage       & Path congestion         & Receiver queue delays  \\
%Network interface type & Number of nodes on path & Congestion window size \\ \bottomrule
%\end{tabular}
%}
%\caption{Network parameters impacting RTT}
%\label{network-parameters}
%\end{table}

The efficiency of MPTCP is mainly dependent on its choice of path scheduler.  In this paper, we argue that the current way of treating the individual subflows by the default and several state-of-the-art schedulers, i.e., practically separately relying only on their TCP level information, is not sufficient. A scheduler's reliance on TCP-level information disables it to fully leverage the available capacity and a more holistic approach to MPTCP and how it manages the connections is needed. 

In this paper, we show via controlled experiments that the MPTCP's default minSRTT scheduler essentially forces the protocol to use only one of the many available flows and thus leads to lower performance.  We develop a novel MPTCP path scheduler, QueueAware,  which exploits hardware device queue occupancy along with TCP RTT for robust and effective scheduling decisions. We implement QueueAware as a modular scheduler in latest stable MPTCP Linux implementation release. We evaluate QueueAware in simulated and real networks for various network configurations and applications such as bulk data transfers, web browsing, web file downloads, video streaming, etc. By comparing QueueAware with minSRTT and several other state-of-the-art schedulers such as DAPS, BLEST, and ECF, we show that our approach outperforms all other schedulers and can adapt to changes in network conditions and background traffic more effectively and efficiently. This results in increased throughput, efficient capacity utilization and better user Quality-of-Experience.

For future work, we intend to investigate the effects of MPTCP path schedulers on several other network factors such as congestion at an access point, over-utilization of channel capacity, queueing delay at receiver etc. We believe that several such network aberrations can be overcome by utilizing network-specific aspects, such as congestion, and receiver-specific parameters (such as window size) etc. Explicitly monitoring, predicting and incorporating these parameters with local network variables and TCP-level information is an interesting research question of its own.


% Sender device queue is one such parameter which needs to be monitored and considered in overall network scheduling decision.
%Only by including cross-layer feedback into MPTCP control loop can we fully exploit the potential offered by multiple connections.
%As shown in the paper, treating the links as independent, parallel TCP flows restrict MPTCP's performance.
%%  This urges MPTCP researchers to contemplate cross-layer feedback
%% loops and external network parameter while scheduling data packets
%% over TCP subflows.
%
%Several other conditions can lead to changes MPTCP's efficiency. Table~\ref{network-parameters} lists few such variables that impact RTT and the network path and which could be exploited by a more holistic MPTCP. These include host-specific parameters, such as device queue length; network-specific aspects, such as congestion, and receiver-specific parameters, such as window size. An efficient MPTCP should look at all or many of these parameters in conjunction while deciding how to schedule the packets and allocate the available flows for data transport.
%
%Several other factors can also significantly impact network behavior. Congestion at an access point, over-utilization of channel capacity, queueing delay at receiver are some such scenarios. However, unlike the locally accessible parameters (such as device queue occupancy), explicitly monitoring and predicting these parameters is an interesting research question of its own. One possibility is to use explicit notifications such as ECN to convey occurrence of such a scenario. Incorporating these mechanisms and comparing its performance impact on current MPTCP implementation would be an interesting future avenue for research in the wider community.
%
%In this paper, we argue that the current way of treating the individual subflows, practically separately relying only on their TCP level information, is not sufficient for fully exploiting the potential offered by multiple connections, and a more holistic approach to MPTCP and how it manages the connections is needed. Our results in this paper illustrate only one small facet of the bigger problem, but broader research efforts are needed to understand better how such multiple connections should be used in modern networks. These cover questions such as fairness to other network flows, general performance issues, flow control, and security issues, but they all apparently require a different approach to the problem than parallel, but largely independent connections.


% \textbf{TODO BELOW}

% . On the host machine itself, along with the device queue length, MPTCP can locally monitor packet send rate of the channel to push more data on flow with higher rate; network packet retries to assess last-mile link quality and current signal strength to predict handovers/link failures and adapt TCP subflow usage accordingly. As shown in the paper,  incorporating such local behavior variables can significantly improve network usage and performance. 

% Several other factors also significantly impact network behavior. Congestion at access point, over-utilization of channel capacity, queueing delay at receiver are some such variables. However, unlike the local stack variables, explicitly monitoring these parameters is an interesting research question. One possibility is to use explicit notifications such as ECN to immediately convey of congestion in the network. Incorporating these mechanisms and comparing its performance impact on current MPTCP implementation would be the focus of our future work.

% Furthermore, several active queue management algorithms such as Random Early Detection (RED), Controlled Delay (CoDel) have been proposed and implemented in Linux over the years \cite{aqmsurvey}. These algorithms aim to handle congestion in device queue by intelligently dropping packets in the buffer. The current MPTCP linux and NS3 implementation does not support these algorithms. However, as such techniques directly influence the number of packets in device queue, its effect on perfromance of QueueAware scheduler would be an interesting aspect in our future work.     


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> realworld_longerDescription.tex <==
\section{Real-World Setup And Experiments}
\label{sec:realexperiments}
\begin{figure}[!t]             
\begin{center}
%\captionsetup{justification=centering}
\includegraphics[width=0.38\textwidth]{Figs/mptcp_testbed}
\caption{Real network experiment setup.}
\label{fig:realsetup}
\end{center}
\end{figure}

%In this section, we validate the performance gains achieved by QueueAware scheduler in real network experiments. 
We assess QueueAware in a real setting using the Linux kernel implementation~\cite{queueawarecode} summarized in Section~\ref{sec:implementation}. Figure \ref{fig:realsetup} shows the test network topology in the University of Helsinki data center. We set up two similar machines with 16 core AMD Opteron processor, 8 GB DDR2 RAM running Ubuntu 16.04 LTS with latest stable MPTCP implementation (version 0.93, based on Linux kernel v4.9.33 \cite{mptcpv93}) as client and server. Both client and server machines are interconnected via two separate Gigabit Ethernet interfaces. One Ethernet connection is routed through the internal University of Helsinki network and therefore sees background traffic from University staff. It has an end-to-end RTT of $>$1ms. The other connection is over a Top-of-Rack (ToR) switch with RTT $<$1 ms.

We compare QueueAware with the following schedulers: (a) minSRTT, (b) Delay Aware Packet Scheduler (DAPS)~\cite{daps}, (c) Blocking Estimation based Scheduler (BLEST)~\cite{blest}, and (iv) Earliest Completion First (ECF)~\cite{ecf}\footnote{For DAPS and BLEST, we use the implementation at \url{https://bitbucket.org/blest_mptcp/nicta_mptcp}. For ECF, we use the implementation at \url{http://cs.umass.edu/~ylim/mptcp_ecf}} \footnote{It must be noted that DAPS, BLEST, and ECF are implemented on MPTCP v0.89 whereas the default minSRTT and our QueueAware scheduler is based on current MPTCP v0.93}. We examine the schedulers on four different real-network workloads: bulk traffic transfer, video streaming, web-file download and adaptability to heterogeneous paths under realistic network conditions for each experiment. We use the  Linux  Traffic Control system (tc) in combination with a Hierarchical Token Bucket (HTB) packet scheduler using Statistical Fair Queuing (SFQ) for network shaping. All our results are averaged over 10 runs unless otherwise mentioned. In between runs, we flush out the TCP cache to ensure that each run is independent of the next.

\subsection{Bulk Traffic}

\begin{figure*}[!t]    
\hspace*{\fill}% 
\begin{center}    
\begin{minipage}[t]{0.243\linewidth}
\vspace{0pt}
\includegraphics[width=0.89\linewidth]{Figs/IFIPGraphs/iPerf-Linux}
\vfill
\caption{Average Throughput Comparison for Bulk Traffic}
\label{fig:iperf_linux}
\end{minipage}
\hfill
\begin{minipage}[t]{0.72\linewidth}
\vspace{0pt}
\begin{subfigure}{0.31\linewidth}
\centering
  \includegraphics[height=4cm, width=4.2cm]{Figs/IFIPGraphs/video-2+2}
  \caption{\label{fig:video-2+2}\textbf{2Mbps+2Mbps}}
\end{subfigure}
\hfill
\begin{subfigure}{0.31\linewidth}
\centering
  \includegraphics[height=4cm, width=4.2cm]{Figs/IFIPGraphs/video-24+16}
  \caption{\label{fig:video-24+16}\textbf{2.4Mbps+1.6Mbps}}
\end{subfigure}
\hfill
\begin{subfigure}{0.31\linewidth}
\centering
  \includegraphics[height=4cm, width=4.2cm]{Figs/IFIPGraphs/video-2+16}
  \caption{\label{fig:video-2+16}\textbf{2Mbps+1.6Mbps}}
\end{subfigure}
\caption{Measured Average Bitrate in Video Streaming for Different Bandwidth Regulations (\textbf{higher is better})}
\label{fig:videoexp}
\end{minipage}
\end{center}    
\hspace*{\fill}% 
\vspace*{-2em}
\end{figure*}

In this section, we compare QueueAware's performance with other schedulers for high application transfer rate over somewhat-homogeneous subflows. The purpose of this experiment is to validate QueueAware's performance improvement for heavily network-dependent applications from simulations. Figure \ref{fig:iperf_linux} shows the average throughput of all schedulers over ten runs.

From the results, it can be observed that QueueAware achieves more than 45\% increase in throughput for bulk traffic over homogeneous paths than DAPS, BLEST and ECF schedulers. QueueAware's performance also supersedes that of default minSRTT scheduler by 37\%. Interestingly, the minSRTT scheduler outperforms DAPS, BLEST, and ECF in the experiment. We attribute minSRTT's efficiency to two reasons. Firstly, DAPS, BLEST and ECF schedulers have been designed to improve MPTCP performance for heterogeneous network path delays wherein BLEST and ECF even goes as far as not sending an available packet on slower subflow and wait for the faster path to become available. For homogeneous subflows, the default scheduler places more number of packets on each path as opposed to BLEST and ECF. Secondly, based on latest MPTCP version minSRTT enjoys several code improvements and optimizations in latest MPTCP kernel unlike DAPS, BLEST and ECF.

\subsection{Video Streaming}

\begin{table}[!t]
\centering
\begin{subtable}{\linewidth}
\centering
\begin{tabular}{llll} 
\toprule
Bandwidth (Mbps) & 2.4 & 2& 1.6  \\
Delay (ms)       & 10  & 20& 30  \\
\bottomrule
\end{tabular}
\caption{Configuration for Video Streaming Experiment}
\label{table:netwvideo}
\end{subtable}

\vspace*{1em}

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{lllll} 
\toprule
Delay (ms)       & 1   & 40& 80& 160    \\
Bandwidth (Mbps) & 950 & 600& 300& 300  \\
\bottomrule
\end{tabular}
\caption{Configuration for Heterogeneous Paths Experiment}
\label{table:netwhetro}
\end{subtable}

\caption{Bandwidth and RTT regulations for experiment setup. Table \ref{table:netwvideo} presents values after both bandwidth and delay shaping whereas \ref{table:netwhetro} shows bandwidth achieved by delay throttling on a 1Gbps ethernet interface}
\end{table}

In this section, we investigate whether QueueAware improves the performance of video streaming applications when compared to other schedulers. We choose streaming as one of our evaluation scenario as it is dominant Internet use case and is widely adopted by content providers such as Netflix, YouTube etc. \cite{streamingapp}. We set up a DASH server and host \textit{Big Buck Bunny} available from a public dataset on it \cite{dashDataset}. We configure the streaming server to provide five representations of the video from 240p to 1080p (same as most content providers).  We re-encode each representation in at least three different bitrates with overall available bit rates from 128Kbps to 3.8Mbps using H.264/MPEG-4 AVC codec. The streaming client employs an Adaptive Bit Rate (ABR) algorithm to download video segments according to available network bandwidth. We throttle our testbed bandwidth to match the bitrates of DASH encodings. Table \ref{table:netwvideo} shows the average delay measured at client-side for each bandwidth configuration. We evaluate scheduler performance when the two subflows are \textit{homogeneous} (2Mbps+2Mbps), \textit{semi-heterogeneous} (2Mbps+1.6Mbps) and \textit{heterogeneous} (2.4Mbps+1.6Mbps). Figure \ref{fig:videoexp} shows the results. 

We observe that QueueAware improves the performance of streaming applications in all network conditions and achieves a closer to ideal bitrate. The performance improvement is more significant in homogeneous and semi-heterogeneous scenarios (8\% and 5\% with default and 10\% and 6\% with ECF respectively) as QueueAware utilizes available paths more efficiently than other schedulers. DAPS yields the worst performance out of all schedulers due to its dependence on RTT ratio of two subflows which provides incorrect results for RTT estimations in Linux. BLEST performance degrades when the paths are heterogeneous whereas QueueAware still achieves the best bitrate in this setting.

\subsection{Web File Download}
\begin{figure}[!t]             
\begin{center}
%\captionsetup{justification=centering}
\includegraphics[width=0.46\textwidth]{Figs/IFIPGraphs/linux-fileDownload}
\caption{Normalized Download Completion Time for Different File Sizes (\textbf{lower is better})}
\label{fig:linux-file-download}
\end{center}
\end{figure}

We now evaluate QueueAware's performance for simple web downloads using \emph{curl}. We set up an Apache 2.2.22 as HTTP server and host varying file sizes ranging from 128KB to 500MB. In order to eliminate application connection time, we only consider the transport-level time to completion in overall completion time. Figure \ref{fig:linux-file-download} presents the average completion time normalized to the maximum achieved value by a scheduler in each file size experiment.

For small web transfers ($<$1MB) all schedulers perform quite similar to each other (it took 0.002s to download a 128KB file by QueueAware vs. 0.003s by minSRTT). This is because for small data transfers, the bandwidth of the primary subflow is more than capable of single shot transmission and thus MPTCP rarely switches to the secondary subflow. Therefore, until the performance of primary subflow degrades during transfer, the choice of the scheduler does not affect the performance of small file downloads. As BLEST and ECF add additional delays by waiting for faster subflow to become available, the default and DAPS scheduler achieve lower completion time for medium file sizes ($\approx$10/100MB). For large files (500MB), BLEST and ECF utilize faster subflow more efficiently than default and DAPS thus achieving a lower completion time. QueueAware always outperforms other schedulers and realizes up to 30\% decrease for medium file sizes and 10\% for large file downloads. 

\subsection{Heterogeneous Path Delays}

\begin{figure}[!t]
\centering
\begin{subfigure}{0.22\textwidth}
\centering
  \includegraphics[height=4cm]{Figs/IFIPGraphs/delay-1_2}
  \caption{\label{fig:delay-1_2}\textbf{40ms+80ms}}
\end{subfigure}%
\hspace{0.7em}
\begin{subfigure}{0.22\textwidth}
\centering
  \includegraphics[height=4cm]{Figs/IFIPGraphs/delay-1_4}
  \caption{\label{fig:delay-1_4}\textbf{40ms+160ms}}
\end{subfigure}
\caption{Average Throughput Comparison for Heterogeneous Path Delays}
\label{fig:delay_linux}
%\vskip -3mm
\end{figure}

We now examine QueueAware's performance for network scenario when subflows have high delay differences such as offered by cellular and WiFi paths. For this experiment, we shape the path delays to emulate two realistic network settings: 
\begin{inparaenum}[i)]
\item when delay on one subflow is twice of the other and,
\item when delay on one subflow is four times of the other subflow.
\end{inparaenum}
The per-path bandwidth for different delay throttling is presented in Table \ref{table:netwhetro}.

Figure \ref{fig:delay_linux} shows the average throughput achieved by all schedulers. For path delay ratio of 2, QueueAware yields an average throughput of 310Mbps which is an improvement of $\approx10\%$ over default scheduler and DAPS and $\approx5\%$ over ECF and BLEST. For network delay ratio of 4, all schedulers perform quite similar to each other as all try to fully utilize the lower delay path to avoid \textit{Head-of-Line blocking} at receiver. In this case, QueueAware still manages to achieve an improvement of $\approx7\%$ over default scheduler and DAPS, and $\approx4\%$ over BLEST and ECF. 


